Recurrent Attention-based Token Selection for Efficient Streaming Video-LLMs

Video Large Language Models (Video-LLMs) excel at understanding videos in-context, provided they have full access to the video when answering queries. However, these models face challenges in streaming scenarios where hour-long videos must be processed online, and questions need timely responses. In this work, we propose a training-free approach compatible with standard Video-LLMs, leveraging three key concepts: 1) LLM-informed selection of visual tokens to identify those that the LLM has attended to and contributed to its understanding of each short clip. Our attention-based selection allows us to discard up to ~95% of unimportant visual tokens with minimal performance loss; 2) Recurrent processing of past selected tokens to generate temporally coherent understanding of each processed clip; 3) Caption-based question answering for lightweight and accurate responses. Our method achieves state-of-the-art performance on streaming video benchmarks, striking a balance between efficiency and effectiveness.

==> algo.tex <==
\begin{algorithm}[H]
\scriptsize
\caption{Streaming Video Processing and Query Answering}
\begin{algorithmic}[1]
\Statex \textbf{Streaming Video Processing}
\State $M_l \gets [\,]$,\quad \texttt{recent\_memory} $\gets$ queue(), \quad \texttt{buffer} $\gets$ [\,]
\State \texttt{MAX\_MEM} $\gets$ 16,\quad \texttt{CLIP\_SIZE} $\gets$ 16

\While{frames available}
    \State \texttt{buffer.append(get\_next\_frame())}
    \If{length(\texttt{buffer}) == \texttt{CLIP\_SIZE}}
        \State \texttt{context} $\gets$ \texttt{recent\_memory + buffer}; \texttt{buffer.clear()}
        \State \texttt{tokens}, \texttt{cap} $\gets$ \texttt{Caption\_and\_Select(context)}
        \If{length(\texttt{recent\_memory}) == \texttt{MAX\_MEM}} \State \texttt{recent\_memory.pop\_left()} \EndIf
        \State \texttt{recent\_memory.append(tokens)}; \quad $M_l$.append(\texttt{cap})
    \EndIf
\EndWhile

\vspace{0.25em}
\Statex \textbf{Query Answering}
\State \texttt{q\_embed} $\gets$ \texttt{embed(query)}
\State \texttt{top\_caps} $\gets$ \texttt{Retrieve\_TopK}(\texttt{q\_embed}, $M_l$)
\State \texttt{context} $\gets$ \texttt{top\_caps} + \texttt{q\_embed}
\State \texttt{answer} $\gets$ \texttt{LLM\_Generate\_Answer(context)}
\end{algorithmic}
\end{algorithm}
